On the Configuration LP for Maximum Budgeted Allocation

We study the Maximum Budgeted Allocation problem, i.e., the problem of selling a set of $m$ indivisible goods to $n$ players, each with a separate budget, such that we maximize the collected revenue. Since the natural assignment LP is known to have an integrality gap of $\frac{3}{4}$, which matches the best known approximation algorithms, our main focus is to improve our understanding of the stronger configuration LP relaxation. In this direction, we prove that the integrality gap of the configuration LP is strictly better than $\frac{3}{4}$, and provide corresponding polynomial time roundings, in the following restrictions of the problem: (i) the Restricted Budgeted Allocation problem, in which all the players have the same budget and every item has the same value for any player it can be sold to, and (ii) the graph MBA problem, in which an item can be assigned to at most 2 players. Finally, we improve the best known upper bound on the integrality gap for the general case from $\frac{5}{6}$ to $2\sqrt{2}-2\approx 0.828$ and also prove hardness of approximation results for both cases.

==> combined-algorithm.tex <==
\section{Combined Algorithm}

In this section we present an algorithm that is a combination of an old algorithm by
Chakrabarty and Goel and Algorithm~\ref{alg:bigitems} presented above. We only solve the case where
all budgets are the same, so they can be assumed to be equal to $1$.

Let $S$ be the set of players that are only incident to the small items $\smallitems_\alpha$. By
Lemma~\ref{lem:partial-budget}, they can be approximated within a factor of $\frac{4-\alpha}{4} >
3/4$ if $\alpha$ is chose to be more than $3/4$. Thus if the weighted fraction of $S$ is big enough,
we can run the original algorithm and get approximation $3/4 + \delta$ for some constant $\delta >
0$.

Otherwise we are going to run Algorithm~\ref{alg:bigitems} which is better when there are many big
items. However, we cannot run the algorithm on $x$ that is the solution to the configuration LP, we
need to preprocess it first to fulfill the assumptions of Algorithm~\ref{alg:bigitems}. We modify
$x$ so that big items are fully assigned and they are alone in their configurations, thus
creating a new solution $x'$. Note that $\Val(x')$ might be smaller than $\Val(x)$, but we prove
that the loss is not too big.

We first change all configurations containing a big item by removing all small items from the
configuration. If there are 2 big items, we pick one of them and remove it as well. After this
step big items are only alone in a configuration.

\comment{This passage about transforming $x$ into $x'$ needs more details and should be more
formal!}
In the second step, we make all big items either fully assigned or not assigned at all. Recall that a
fully assigned item $j$ has $\sum x_{ij} = 1$. First get rid
of all the cycles with big items. Take a cycle and move some probability on the cycle in some
direction, so that one edge disappears from the cycle. Thus we can assume that there are no cycles,
only trees.

Now in the trees we shift the weights around, so that all the big items are fully assigned, possibly
getting rid of small configurations in favor of big items. We take a big item $j$ that is not fully assigned and look at the 2
subtrees in both directions. In both subtrees there should be enough total space to accommodate for
item $j$ by taking a path in the subtree to a leaf and moving weights towards the leaf along the
path.

Let us denote the new solution $x'$. We have that all big items are either fully assigned or not
assigned in $x'$ and all are alone in their configurations. Also, big items never form a cycle. Thus,
we can now run Algorithm~\ref{alg:bigitems}.

Let $\players_B$ be the set of players that have at least one configuration with a big item and
$\players_S = \players \setminus \players_B$, i.e.\ players with only small configurations.
Let $\Val_B (x) = \sum_{i\in \players_B} \Val_i(x)$ and $\Val_S (x) = \sum_{i\in \players_S}
\Val_i(x)$, i.e.\ the sum of $\Val_i (x)$ restricted to sets $\players_B$ and $\players_S$.
We use the shortcuts $V_B = \Val_B (x)$ and $V_S = \Val_S (x)$. Note that $V_B + V_S = \Val(x)$.

When considering solution $x'$, we pretend that all big items have price 1, i.e.\ their price is
equal to the budget. We denote this scaled up instance by $\instance'$. Furthermore, let $E_B =
\sum_{i \in \players_B, j \in \bigitems} x'_{i, \{j\}}$ and $E_S = \sum_{i \in \players,
\conf\subseteq \smallitems} x'_{i, \conf} w(\conf)$, i.e.\ the total value of configurations of big
items and small items for $x'$ in $\instance'$. Note that $\Val^{\instance'}(x') = E_B + E_S$.

\comment{Would it be better to have $\Val_B$ instead of $V_B$?}

\begin{theorem}
  There is a polynomial algorithm that assigns total value of
  $$\frac{3}{4} \Val(x) + \frac{\alpha - 0.75}{2} V_B.$$
  \label{thm:random-alg}
\end{theorem}

\begin{proof}
  We first transform $x$ into $x'$ as described above and then run Algorithm~\ref{alg:bigitems},
  which by Theorem~\ref{thm:algbigitems} returns a solution $x^*$ with value $\Val (x^*)$ at least
  $\alpha E_B + \frac{3}{4} E_S$. We show that
  $\Val (x^*)$ is at least $\frac{3}{4} \Val(x) + \frac{\alpha - 0.75}{2} V_B$.

  We have that $E_S = V_S + V_B^\smallitems$, where $V_B^\smallitems = \sum_{i \in \players_B,
  \conf\subseteq \smallitems} x'_{i, \conf} w(\conf)$, i.e.\ the total value of small configurations
  for $\players_B$. Let $r$ be the total probability corresponding to small configurations in $x'$
  for $\players_B$, i.e.\ $r = \sum_{i \in \players_B, \conf\subseteq \smallitems} x'_{i, \conf}$.
  Note that $E_B = |\players_B| - r$ and $r$ is at most $|\players_B| / 2$, since all big items are
  assigned and they form a forest.

  $\Val_S (x^*)$ is the value assigned by Algorithm~\ref{alg:bigitems} to $\players_S$ and we have
  $\Val_S (x^*) \ge \frac{3}{4} V_S$. In the remaining part of the proof we focus on the players in
  $\players_B$ and their corresponding quantity $\Val_B (x^*)$. We prove that $\Val_B (x^*) \ge V_B
  (3/4 + \frac{\alpha - 0.75}{2})$. By Theorem~\ref{thm:algbigitems}, the players in $\players_B$
  are assigned at least $\Val_B (x^*) \ge \alpha E_B + \frac{3}{4}V_B^\smallitems = \alpha
  (|\players_B| - r) + \frac{3}{4}V_B^\smallitems$.

  Let
  $$q = \frac{V_B - V_B^\smallitems}{|\players_B| - r},$$
  i.e.\ the average weight of configurations in $x$ that are not the small configurations counted in
  $V_B^\smallitems$. The same average, but taken for $x'$ is at least $\alpha$, so we have $q \ge
  \alpha$, because otherwise $x'$ would be a better solution than $x$ which is a contradiction.

  We can write
  $$\Val_B (x^*) \ge \frac{\alpha}{q} (V_B - V_B^\smallitems) + \frac{3}{4} V_B^\smallitems,$$
  since
  $$\alpha (|\players_B| - r) = \frac{\alpha}{q} (V_B - V_B^\smallitems).$$

  We have $q \le 1$, so $\frac{\alpha}{q} > \frac{3}{4}$. If we could upper bound $V_B^\smallitems$
  by a constant fraction of $V_B$, it would imply approximation better than $3/4$. Recall that
  $V_B^\smallitems \le r$. Let us fix $\alpha$ and $q$. We now upper bound the ratio
  $V_B^\smallitems / V_B = \frac{V_B^\smallitems}{V_B^\smallitems + q(|\players_B| - r)}$. For a
  fixed $q$, such that $\alpha \le q \le 1$, $V_B^\smallitems / V_B$ is maximized when
  $V_B^\smallitems$ is maximized, so $V_B^\smallitems = r$. Hence we have
  $$\Val_B (x^*) \ge V_B \left(\alpha \frac{(|\players_B| - r)}{r + q (|\players_B| - r)} +
  \frac{3}{4} \cdot \frac{r}{r + q(|\players_B| - r)} \right).$$

  For fixed $r$ and $\alpha$, the expression above is maximized when $q$ is maximized, so $q =
  1$. Since $r \le |\players_B| / 2$, we finally get
  $$\Val_B (x^*) \ge \frac{V_B}{2} \left(\alpha + \frac{3}{4}\right) = \frac{3}{4} V_B + \frac{\alpha - 0.75}{2}
  V_B$$
  and thus $\Val (x^*) \ge \frac{3}{4} \Val(x) + \frac{\alpha - 0.75}{2} V_B$.
\end{proof}


\begin{corollary}
  Combining Theorem~\ref{thm:random-alg} and the algorithm of Chakrabarty and Goel gives
  value at least
  $$\frac{3}{4} \Val(x) + \max\left\{\frac{\alpha - 0.75}{2} V_B,\quad
  \frac{1 - \alpha}{4} V_S\right\}.$$
  For $\alpha = 0.853553$ the algorithm assigns value at least $0.77145 \Val(x)$.

  \label{cor:combined-algorithm}
\end{corollary}

\begin{proof}
  The worst approximation ratio is achieved when
  $$\frac{\alpha - 0.75}{2} V_B = \frac{1 - \alpha}{4}V_S.$$

  Let $y = V_B / \Val(x)$, then $1 - y = V_S / \Val(x)$, since $\Val(x) = V_S + V_B$. We thus have
  $$\frac{\alpha - 0.75}{2} y = \frac{1 - \alpha}{4}(1 - y),$$
  which implies
  $$y = \frac{2 (1 - \alpha)}{2 \alpha - 1}.$$

  The optimal $\alpha$ is such that it maximizes the function
  $$\frac{(\alpha - 0.75)(1 - \alpha)}{(2\alpha - 1)}$$
  on the interval $(3/4, 1]$. Hence $\alpha \approx 0.853553$ is the optimal value and gives approximation
  ratio $0.77145$.
\end{proof}


==> proofs.tex <==
\section{Proofs of various lemmas}
\label{sec:proofs}

\subsection{Proof of Lemma \ref{lem:buckets}}
\setcounter{restatecounter}{\ref{lem:buckets}}
\addtocounter{restatecounter}{-1}
\begin{restatement}
  Let $x$ be the solution to the assignment LP, $i\in \players$ and let $\alpha \ge 1$ be such that
  $\Val_i(x) = B_i / \alpha$. Let $a_1$ be the average price of items in the first bucket of player
  $i$, i.e.\ $a_1 = \sum_j x'_{bj} p_{bj}$, where $b$ is the first bucket. Let $r_1$ be the average
price
  of items in the first bucket of price more than $\alpha a_1$. Then
  $$\Alg_i(x) \ge \Val_i(x) \left(1 - \frac{r_1}{4 B_i}\right).$$
  In particular, since $r_i \le B_i$, Algorithm~\ref{alg:buckets} gives a 3/4-approximation.

\end{restatement}
\begin{proof}
  The expected value of the solution $x^*$ for player $i$ is $\EX[\Val_i (x^*)] = \Val_i (x)$,
  because the probability of assigning item $j$ to player $i$ is $x_{ij}$. The problem with the
  assignment $x^*$ is that some players might go over the budget, so we cannot make use of the full value
  $\Val_i (x^*)$. We now prove that we only lose $\frac{r_1}{4 B_i}$-fraction of $\Val_i(x)$ by
  going over the budget of player $i$.

  Note that $\alpha \ge 1$, since a solution to assignment LP never goes over the budget $B_i$. Let
  $a_b$ be the average price in bucket $b$. The matching picks at most one item from each bucket and
  suppose from each bucket $b$ it picks item of price more than $\alpha \cdot a_b$. Then since
  $\alpha \sum a_b =
  B_i$, the player would be assigned more than her budget. However, if we assume that all items
  within $b$-th bucket have price at most $\alpha \cdot a_b$, all maximum matchings assign price at
  most $B_i$ to player $i$. We thus define $p'_{bj}$ to be $\min\{p_{bj}, \alpha \cdot a_b\}$ and we
  get a new instance $\instanceJ$ with prices $p'$ and buckets become the players of this instance.
  From the previous discussion we know no player goes over budget when using the fictional prices
  $p'$, so $\Val_i ^ \instanceJ (x^*) \le B_i$. Thus $\Alg_i(x)$ can be lower-bounded by
  $\EX[\Val_i^\instanceJ (x^*)] = \Val_i^\instanceJ (x')$. We now prove that $\Val_i^\instanceJ (x')
  \ge (1 - \frac{r_1}{4 B_i}) \Val_i (x)$.

  Let $r_b$ be the average price of items in bucket $b$ with price above $\alpha \cdot a_b$ and let
  $q_b$ be the average price of the rest of the items in bucket $b$. Note that $q_b \ge r_{b +
  1}$. We let $x'_b$ be the probability corresponding to
  $r_b$, i.e.\ the sum of all $x'_{bj}$ where $p_{bj} > \alpha \cdot a_b$. Since $p_{ij}$ is changed
  to $\alpha \cdot a_b$ in $p'$ for these items, the
  difference in price for bucket $b$ is $(r_b - \alpha a_b) x'_b$. The loss of value by going from
  $p$ to $p'$ is thus
  $$\Val_i (x) - \Val_i ^ \instanceJ (x') = \sum_b (r_b - \alpha a_b) x'_b.$$

  Since $a_b = (r_b - q_b) x'_b + q_b$, we have $(r_b - \alpha a_b) x'_b = (r_b - \alpha q_b)x'_b -
  (r_b - q_b) \alpha {x'_b}^2 \le (r_b - q_b) (x'_b - \alpha {x'_b}^2)$
  where the last inequality follows from $\alpha \ge 1$. Since $q_b \ge r_{b + 1}$, we get $(r_b -
  \alpha a_b) x'_b \le (r_b - q_b) (x'_b - \alpha {x'_b}^2) \le (r_b - r_{b + 1}) (x'_b - \alpha
  {x'_b}^2)$. It follows that
  \begin{equation*}
    \Val_i (x) - \Val_i ^ \instanceJ (x')
    \le \sum_b (r_b - r_{b + 1}) (x'_b - \alpha {x'_b}^2).
  \end{equation*}

  The maximum of $x'_b - \alpha {x'_b}^2$ is attained for $x'_b = \frac{1}{2 \alpha}$ and we get
  \begin{equation*}
    \Val_i (x) - \Val_i^\instanceJ (x') \le \sum_b \frac{r_b - r_{b + 1}}{4 \alpha} \le
    \frac{r_1}{4 \alpha} % \le \frac{p_{max}}{4 \alpha}
  \end{equation*}

  Hence $$\Alg_i(x) \ge \Val_i^\instanceJ (x') \ge \Val_i(x) - \frac{r_1}{4\alpha} = \Val_i (x)
  \left(1 - \frac{r_1}{4 B_i}\right)$$
  which concludes the proof.
\end{proof}

\subsection{Proof of Lemma \ref{lem:projection}}
\setcounter{restatecounter}{\ref{lem:projection}}
\addtocounter{restatecounter}{-1}
\begin{restatement}
  Let $y$ be a well-structured solution to the configuration LP. Then there exists a solution $x$ to
  the assignment LP with $\Val_i(x) = \Val_i(y)$ such that
  \begin{equation*}
    \sum_{\conf \subseteq \items}|\bigitems \cap \conf|\cdot y_{i, \conf} \in
      \left[\frac{1-\delta}{2}, \frac{1+\delta}{2}\right]
    \Leftrightarrow
    \sum_{j: j \in \bigitems} x_{ij} \in \left[\frac{1-\delta}{2}, \frac{1+\delta}{2}\right]
  \end{equation*}
  for all $i \in \players$. Furthermore, $x$ can be produced from $y$ in polynomial time.
\end{restatement}
\begin{proof}
  Note that we can assume that each configuration in $y$ contains at most 2 big items. If a
  configuration contains more than 2 big items, all but 2 big items can be removed without
  decreasing the objective value, since $2(1 - \beta) \ge 1$ and thus the configuration remains over
  the budget.

  We first modify $y$ to a new solution $y'$ where each player does not have at the same time
  a configuration with 2 big items and a configuration with no big items. Solution $y'$ is then
  projected to a solution $x$ to the assignment LP with desired properties.

  Fix player $i$ and two configurations $\conf, \conf'$ such that $\conf$ contains two big items and
  $\conf'$ contains no big items. We can assume that $y_{i\conf} = y_{i\conf'}$, otherwise we can
  split the bigger fractional value into two and disregard one of them. We want to move the second big
  item from $\conf$ into $\conf'$ without decreasing the objective value. This is done by moving
  back small items from $\conf'$.

  Let us order the items in $\conf'$ by value in decreasing order $j_1, \dots, j_k$. We move a
  big item from $\conf$ to $\conf'$ and then move $j_1, j_2, \dots$ to $\conf$ until it has
  profit at least 1 or we run out of items. Let $F$ and $F'$ be the transformed configurations which
  arise from $\conf, \conf'$ respectively.

  If the value of $\conf'$ is less than $\beta$, then we run out of items and the value of $F$ is at
  least $1-\beta + \sum_{j\in\conf'} p_j$ and the value of $F'$ is at least $1-\beta > \beta$, so the objective
  value improved and $y$ is not an optimal solution, a contradiction. Hence we have that the value
  of $\conf'$ is at least $\beta$ and $F$ has value at least $1$.

  It remains to prove that the value of $F'$ is at least as big as the value of $\conf'$. In the
  above process we move a big item of value at least $1-\beta$ to $F'$ and we now show that we
  move less in the other direction. Suppose towards contradiction that we moved more than $1-\beta
  \ge 2\beta$ to $F$, then we moved at least 2 small items and the last item added must have been of
  value at least $\beta$. But then only one such item is necessary, since $\conf$ already contains a
  big item that has value of at least $1-\beta$.

  Applying this procedure whenever we can, we end up with a modified solution $y'$ to the
  configuration LP in which there is no player at the same time having a configuration containing
  two big items and a configuration with no big items. Also, $y'$ is such that
  \begin{equation*}
    \sum_{\conf \subseteq \items}|\bigitems \cap \conf|\cdot y_{i, \conf} =
    \sum_{\conf \subseteq \items}|\bigitems \cap \conf|\cdot y'_{i, \conf},
  \end{equation*}
  because big items are only moved between configurations, so their contribution to the sums above
  is preserved.

  The pairs of configurations $\conf, \conf'$ can be chosen in such a way that we only create
  polynomially many new configurations in total. To see this, let $T = \{\conf_1, \dots, \conf_k\}$ be
  the configurations in $y$ that have two big items and let $S = \{\conf'_1, \dots, \conf'_\ell\}$ be
  the configurations in $y$ with no big items. We process $T$ one by one. For each $\conf_j \in T$
  we try to move the second big item to the configurations $\conf'_1, \dots, \conf'_\ell$ one by
  one. In the end
  we try at most $k\cdot \ell$ different pairs and each pair creates at most 2 new configurations.
  Since $k\cdot \ell$ is polynomial in the size of the instance, also the number of new
  configurations is polynomial.

  Now we project $y'$ to a solution $x$ to the assignment LP as follows: for every player $i$ and
  configuration $\conf$, consider the items in $\conf$ in non-increasing order according to
  $p_{ij}$. If the total value of $\conf$ is at most $B_i$, the configuration $\conf$ contributes
  $y'_{i\conf}$ to the value $x_{ij}$ for all items $j \in \conf$. Otherwise the total value goes
  over the budget and only the first part of the ordered items that is below the budget gets
  contribution $y'_{i\conf}$ and the rest of the items gets contribution 0, except the one item that
  is only partially below the budget which gets some fraction between $0$ and $y'_{i\conf}$. In
  particular this means that big items get the full contribution $y'_{i\conf}$.

  Let us now formalize the intuition given above.
  Let $j'$ be the minimum index such that $\sum_{1\leq j\leq j'} p_{ij}>B_i$. For all
  $j>j'$, set $z_{ij\conf}=0$, for all $j<j'$ set $z_{ij\conf}=y'_{i\conf}$ and set
  $$z_{ij'\conf}=\frac{B_i-\sum_{1\leq j< j'} p_{ij}}{p_{ij'}} y'_{i\conf}.$$
  Finally, we define
  $$x_{ij} = \sum_{\conf \subseteq \items} z_{ij\conf}.$$

  We have $\Val(x) = \Val(y') = \Val(y)$, since $\sum_{j} z_{ij\conf}p_{ij} = w_i(\conf)
  y_{i\conf}$, i.e.\ the contribution of each configuration is preserved by the projection.

  The projection from $y'$ to $x$ gives full contribution $y'_{i\conf}$ to the largest item in $\conf$.
  If there are two big items in $\conf$, the second big item does not get the full contribution.
  However, this happens only when $\sum_{\conf \subseteq \items}|\bigitems \cap \conf|\cdot y'_{i,
  \conf} > 1$ and in this case all configurations in $y'$ for player $i$ have a big item. Then $1
  \le \sum_{j: j \in \bigitems} x_{ij}$. However, if the total weight of big items in $y'$ for
  player $i$ is less than 1, the same total weight is projected on $x$. We thus have
  \begin{equation*}
    \sum_{j: j \in \bigitems} x_{ij} =
    \sum_{\conf \subseteq \items}|\bigitems \cap \conf|\cdot y_{i, \conf}
  \end{equation*}
  if $\sum_{\conf \subseteq \items}|\bigitems \cap \conf|\cdot y_{i, \conf} \le 1$ and otherwise
  $\sum_{j: j \in \bigitems} x_{ij} > 1$. This concludes the proof.
\end{proof}

\subsection{Proof of Lemma \ref{lem:not-fully-assigned}}
\setcounter{restatecounter}{\ref{lem:not-fully-assigned}}
\addtocounter{restatecounter}{-1}
\begin{restatement}
  Let $\epsa>0$ be a small constant and consider player $i$ such that $\Val_i (x) \leq
  1-\epsa$. Then
  $\Alg_i (x) \ge \frac{3+\epsa/5}{4} \Val_i(x)$.
\end{restatement}
\begin{proof}
For player $i$, select the largest $Q_i$ such that
\begin{equation*}
Q_i = \sum_{j} x_{ij} q_{ij}, \qquad \mbox{ where } q_{ij} = \min\{p_{ij}, Q_i\}.
\end{equation*}

Note that such a $Q_i$ always exists, since $0$ always satisfies the equation. Let $f_i(z) =
\sum_{j} x_{ij} \min\{p_{ij}, z\}$ and note that $f_i(z)$ is a continuous function. We have
$f_i(1) = \Val_i(x) < 1$ and $f_i(0) = 0$ and we want to find the largest $Q_i$, such that $f_i(Q_i) = Q_i$.

If we substitute prices $p_{ij}$ with $q_{ij} = \min\{p_{ij}, Q_i\}$, the ordering of the items for
a player by the price stays the same. Thus Algorithm~\ref{alg:buckets} produces the same result no
matter which one of the two prices we use. Let $D_i$ denote the difference $\sum_j x_{ij} (p_{ij} -
q_{ij}) = \Val_i(x) - Q_i$. We do case distinction based on the size of~$D_i$.

\begin{description}
  \item[Case $D_i > \frac{\epsa}{5} \Val_i(x)$:]\hfill\\
  By Lemma~\ref{lem:buckets}, if we run Algorithm~\ref{alg:buckets} on $x$ but use values $q_{ij}$
  and budget $Q_i$ in the analysis, we get $\Alg_i(x) \ge \frac{3}{4} Q_i$. In order to improve this
  we use the fact that $q_{ij} < p_{ij}$ only for at most one unit of the largest items. If already
  more than one unit of items is at least $Q_i$, then we have $f_i(Q_i) > Q_i$. Since $f_i(1) < 1$
  and $f_i$ is continuous, $Q_i$ is not the largest solution to $f_i(z) = z$, a contradiction.

  Moreover, since the assignment according to the analysis with respect to $q$ does not violate the
  budget $Q_i$, we can always add back the difference $p_{ij} - q_{ij}$ if $j$ is assigned to $i$
  without violating the budget $B_i$, since $p_{ij} - q_{ij} \le B_i - Q_i$. We are not
  losing a quarter from the difference $D_i$, so we have an advantage of $D_i / 4 > \frac{\epsa}{20}
  \Val_i(x)$. Formally, the expected profit is
  \begin{equation*}
  \frac{3}{4}Q_i + D_i = \frac{3}{4}(Q_i + D_i) + D_i/4 = \frac{3}{4} \Val_i(x) + D_i/4,
  \end{equation*}
  which is at least $\left(\frac{3}{4} + \frac{\epsa}{20}\right) \Val_i (x)$.

  \item[Case $D_i \leq \frac{\epsa}{5} \Val_i(x)$:]\hfill\\
  In this case we apply Lemma~\ref{lem:buckets} with prices $q$ and budget $1$. Now since $Q_i$ is
  bounded away from $1$, $\Alg_i(x)$ is more than $3/4Q_i$. Formally,
  \begin{equation*}
  \Alg_i(x) \ge (1 - Q_i/4) Q_i = (1 - Q_i/4) \Val_i (x) - (1 - Q_i/4)D_i \geq (1 - Q_i/4) \Val_i
  (x) - D_i.
  \end{equation*}
  As $Q_i \leq \Val_i (x) \le 1-\epsa$,
  \begin{equation*}
  \Alg_i(x) \ge \left(1- \frac{1-\epsa}{4}\right) \Val_i (x) - D_i
  \geq \left(1- \frac{1-\epsa/5}{4}\right) \Val_i (x) = \frac{3+\epsa/5}{4} \Val_i (x).
  \end{equation*}
\end{description}

\end{proof}

\subsection{Proof of Lemma \ref{lem:non-half}}
\setcounter{restatecounter}{\ref{lem:non-half}}
\addtocounter{restatecounter}{-1}
\begin{restatement}
  Let $\delta > 0$ be a small constant, $\beta$ be such that $\delta / 4 \le \beta$ and consider a
  player $i$ such that $\Val_i(x)
  \geq 1 - \delta^2 / 8$ and $\sum_{j: j \in \bigitems} x_{ij} \not \in \left[\frac{1-\delta}{2},
  \frac{1+\delta}{2}\right]$. Then
  $\Alg_i(x) \ge \frac{3 + \delta^2/64}{4} \Val_i(x)$.
\end{restatement}
\begin{proof}
If the average in the first bucket is more than $\frac{3 + \delta^2/64}{4} \Val_i(x)$ then we are
done, since assigning a random item from that bucket gives sufficient profit.
If
$r_1 \leq 1-\delta^2 / 16$, Lemma~\ref{lem:buckets} already implies the claim. Therefore assume from
now on that $r_1 \ge
1-\delta^2/16$ and $r_2 \le \frac{3 + \delta^2/16}{4}$, so $r_1 - r_2 \geq 1/8$, since $\delta$ is
small.

Select $\alpha \ge 1$ such that $\Val_i(x) = 1/\alpha$. In the proof of Lemma~\ref{lem:buckets} we
have that the expected decrease in value compared to $\Val_i (x)$ in our rounding is at most
$$
\sum_b (r_b - r_{b+1})(x'_b - \alpha {x'_b}^2).
$$

This can be rewritten as
\begin{align*}
(r_1 - r_2) (x'_1 - \alpha {x'_1}^2) + \sum_{b\geq 2} (r_b - r_{b+1})(x'_b - \alpha {x'_b}^2)
&\leq (r_1 - r_2) (x'_1 - \alpha {x'_1}^2) + (r_2 - r_n) \cdot \frac{1}{4 \alpha}\\
&\leq 1/8 (x'_1 - \alpha {x'_1}^2) + 7/8 \cdot \frac{1}{4 \alpha}.\\
\end{align*}
The last inequality follows from $(x'_1 - \alpha {x'_1}^2) \le \frac{1}{4\alpha}$ and $r_1 - r_2\ge
1/8$.

We now prove that $x'_1$ can not be close to $1/2$. The probability $x'_1$ corresponds to items in the
first bucket that have value at least $\alpha a_1$. Suppose towards contradiction that more than
$\delta^2 / (16 \beta)$-fraction of these items are not big items, so they have value at most $1 - \beta$.
Then $r_1 < 1 - \frac{\delta^2}{16 \beta}\cdot \beta = 1 - \delta^2 / 16$, a contradiction. This means
that $x'_1 = (\sum_{j \in \bigitems} x_{ij}) + \gamma$, where $\gamma \in [0, \delta^2/(16\beta)]$.
By $\beta \ge \delta / 4$, $\gamma \in [0, \delta / 4]$. Since $\sum_{j \in \bigitems} x_{ij}
\not\in \left[\frac{1-\delta}{2}, \frac{1+\delta}{2}\right]$, we have $x'_1 \not\in
\left[\frac{1-\delta/2}{2}, \frac{1+\delta/2}{2}\right]$.

We now use the fact that $x'_i$ is bounded away from $1/2$ to prove that the loss in the rounding is
less than $1/4$. For function $z-z^2$ the maximum is attained for $z=1/2$, so $z$ bounded away from
$1/2$ by gives values bounded away from maximum which is 1/4. For function $z-\alpha z^2$ the
maximum is attained very close to $1/2$ provided that $\alpha$ is close to $1$. Again, $z$ bounded
away from $1/2$ gives values bounded away from the maximum. In the rest of the proof we formalize
this intuition.

The maximum for the
function $z(1 - \alpha z)$ is attained for $z = \frac{1}{2 \alpha}$ and we can prove that
$\frac{1}{2 \alpha} \in \left[\frac{1-\delta/2}{2}, \frac{1+\delta/2}{2}\right]$. Since $\alpha \ge 1$,
it only remains to prove that $\frac{1}{2 \alpha} \ge \frac{1 - \delta/2}{2}$. By $1 / \alpha \ge
1 - \delta^2 / 8$,
$$\frac{1}{2 \alpha} \ge \frac{1 - \delta^2 / 8}{2} > \frac{1 - \delta/2}{2}.$$

The function $z - \alpha z^2$ is symmetric around $\frac{1}{2 \alpha}$ and this value is closer to
the beginning of the interval $\left[\frac{1-\delta/2}{2}, \frac{1+\delta/2}{2}\right]$, so the
maximum of $x'_1 - \alpha {x'_1}^2$ is attained when $x'_1 = \frac{1 - \delta/2}{2}$.

We have that
$$x'_1 - \alpha {x'_1}^2 \le x'_1 - {x'_1}^2 = \frac{1 - \delta^2/4}{4} \le \frac{1}{4}{(1 - \delta^2 /
8)}^2.$$

Since $1 - \delta^2 / 8 \le \frac{1}{\alpha}$,
$$x'_1 - \alpha {x'_1}^2 \le \frac{1 - \delta^2 / 8}{4 \alpha}.$$

We can finally bound the decrease in our rounding to be at most
$$
r_1 \left(\frac{1}{8} \cdot \frac{1-\delta^2 / 8}{4 \alpha} + \frac{7}{8} \cdot \frac{1}{4
\alpha}\right) = \frac{r_1 (1 -\delta^2/64)}{4 \alpha}.
$$
The claim follows from the fact that $r_1 \le 1$.
\end{proof}

\subsection{Proof of Lemma~\ref{lem:non-wellstruct}}
\setcounter{restatecounter}{\ref{lem:non-wellstruct}}
\addtocounter{restatecounter}{-1}
\begin{restatement}
  Given a solution $y$ to the configuration LP which is not $(\epsilon, \delta)$-well-structured and
  $\beta \ge \delta / 4$, we can in polynomial time find a solution with expected value at least
  $\frac{3 + \epsilon \delta^2 / 64}{4}\Val(y)$.
\end{restatement}
\begin{proof}
  Let $x$ be a solution to the assignment LP produced from $y$ as in Lemma~\ref{lem:projection}.
  Then more than weighted $\epsilon$-fraction of players have $\sum_{j: j \in \bigitems} x_{ij} \not\in
  \left[\frac{1-\delta}{2}, \frac{1+\delta}{2}\right]$.

  According to Lemma~\ref{lem:not-fully-assigned} using $\epsilon' = \delta^2 / 8$, we have
  $\Alg_i(x) \geq \frac{3 + \delta^2 / 40}{4} \Val_i(x)$ if $\Val_i(x) \leq 1 - \delta^2 / 8$. By
  Lemma~\ref{lem:non-half}, using $\beta \ge \delta / 4$ implies $\Alg_i(x) \geq \frac{3 + \delta^2 / 64}{4}
  \Val_i(x)$ if $\Val_i(x) \geq 1-\delta^2 / 8$ and $\sum_{j: j \in \bigitems} x_{ij} \not\in
  \left[\frac{1-\delta}{2}, \frac{1+\delta}{2}\right]$. Hence for weighted $\epsilon$-fraction of
  players we get $\Alg_i(x) \geq \frac{3 + \delta^2 / 64}{4} \Val_i(x)$, so the total gain is at
  least $\frac{3 + \epsilon\delta^2 / 64}{4} \Val(y)$.
\end{proof}

\subsection{Proof of Lemma~\ref{lem:min-wellstruct}}
\setcounter{restatecounter}{\ref{lem:min-wellstruct}}
\addtocounter{restatecounter}{-1}
\begin{restatement}
For every $j\in \smallitems$, $\EX_T  \left[ \min \left[1, \sum_{i \in \players_j \cap T} 2x'_{ij}
\right]\right] \geq (1-\delta) \frac{3}{4}
  \sum_{i\in \players_j} x_{ij}$.
\end{restatement}
\begin{proof}
We slightly abuse notation and also denote by $T$ the event that the players in $T\subseteq
\players$ were those that were not assigned big items. Let also $x(T) = \min \left[1, \sum_{k \in
\players_j \cap T} 2x'_{kj} \right]$ for the considered small item $j$. With this notation,
$$
\EX_T  \left[ \min \left[1, \sum_{i \in \players_j \cap T} 2x'_{ij} \right]\right] = \sum_{T
  \subseteq \players} \Pr[T] \cdot x(T).
$$
We shall show that we can lower bound this quantity by assuming that $j$ is only fractionally
assigned to two players. Indeed, suppose that $j$ is fractionally assigned to more than two players.
Then there must exist two players, say $i$ and $i'$, so that $0 <x'_{ij} <
1/2$ and $0 < x'_{i'j}<1/2$; the fractional assignment of a small item to some player never
exceeds $1/2$ by construction of $y'$ and $x'$.
We can write $\sum_{T
  \subseteq \players}\Pr[T] \cdot x(T)$ as
\begin{align}
\label{eq:summy}
\sum_{T  \subseteq \players \setminus \{i,i'\}} ( &\Pr[T] \cdot x(T) + \Pr[T \cup \{i\}] \cdot
  x(T \cup \{i\}) + \Pr[T \cup \{i'\}] \cdot
  x(T \cup \{i'\}) \\
\nonumber & +  \Pr[T \cup \{i,i'\}] \cdot
  x(T \cup \{i,i'\}))
\end{align}
Note that if we shift some amount of fractional assignment from $x_{ij}$ to $x_{i'j}$ (or
vice-versa) then $x(T)$ and $x(T \cup \{i,
i'\})$ do not change. We shall now analyze the effect such a shift has on the sums $\sum_{T
  \subseteq \players \setminus \{i,i'\}}   \Pr[T \cup \{i\}] \cdot
  x(T \cup \{i\})$ and  $\sum_{T
  \subseteq \players \setminus \{i,i'\}}   \Pr[T \cup \{i'\}] \cdot
x(T \cup \{i'\})$.
Note that after this shift $x'$ might not be a valid solution to the assignment LP, namely we might
go over the budget for some players. However, our goal is only to prove a lower-bound on
$\EX[\Val(x^{(2)}]$.

For this purpose let $F_i$ denote the probability that the set $T$ is selected such that the value
of
$x(T\cup \{i\})$ is strictly less than $1$, i.e.,
$$
F_i := \sum_{T
  \subseteq \players \setminus \{i,i'\} : x(T \cup \{i\}) < 1}   \Pr[T \cup \{i\}].
$$
Similarly we define $G_i$ for sets where $x(T\cup \{i\})$ is exactly 1, i.e.,
$$
G_i := \sum_{T
  \subseteq \players \setminus \{i,i'\} : x(T \cup \{i\}) = 1}   \Pr[T \cup \{i\}].
$$
The definition of $F_{i'}$ and $G_{i'}$ is analogous. Note that if we, on the one hand, decrease
$x_{ij}$ by a small $\eta$ and increase $x_{i'j}$ by $\eta$, this changes~\eqref{eq:summy} by $\eta
(-F_i - G_i + F_{i'})$. On the other hand, if we increase $x_{ij}$ and decrease $x_{i'j}$ by $\eta$,
then~\eqref{eq:summy} changes by $\eta (F_i - F_{i'} - G_{i'})$. We know that one of $\eta(F_i -
F_{i'})$ and $\eta(-F_i + F_{i'})$ is non-positive,
so either $\eta (-F_i - G_i + F_{i'})$ or $\eta (F_i - F_{i'} - G_{i'})$ are non-positive as well.

After the small change by $\eta$, $F_i$ increases by $G_i$ or $F_{i'}$ by $G_{i'}$, so further
changes in the same direction will be also non-positive. We can therefore either shift fraction of
$x_{ij}$ to $x_{i'j}$ (or
vice versa) without increasing~\eqref{eq:summy} until one of the variables either becomes $0$ or
$1/2$. If it becomes $0$ then we repeat  with one less fractionally assigned small item and if it
becomes
$1/2$ then we repeat by considering two other players where $j$ is fractionally assigned strictly
between $0$ and $1/2$.

By repeating the above process, we may thus assume that $j$ is fractionally assigned to at most
two players say $1$ and $2$ and $x'_{1j}, x'_{2j} \leq 1/2$. We therefore have that \eqref{eq:summy}
is equal to
$$
\Pr[ 1,2 \not \in T] \cdot 0  + \Pr[ 1 \in T, 2 \not \in T]\cdot  2x_{1j} + \Pr[
1
\not \in T, 2 \in T]\cdot  2x_{2j} + \Pr[1, 2\in T] \cdot \min[ 1, 2x_{1j} +2x_{2j}]
$$

It is clear that the above expression is minimized whenever $ \Pr[1, 2\in T]$ is maximized;
however, since our distribution over the assignments of big items is negatively correlated and it
preserves
the marginals (which are at most $(1+\delta)/2$), it holds that $ \Pr[1, 2\in T]\leq
\frac{(1-\delta)^2}{4}$(since the worst case is that $\Pr[1\in T]=\Pr[2\in T]=\frac{1-\delta}{2}$),
and hence one can see that the above expression is at least
$$
\left(\frac{1-\delta}{2}-\frac{(1-\delta)^2}{4}\right)2x_{1j}+\left(\frac{1-\delta}{2}-\frac{
\left(1-\delta\right)^2}{4}\right)2x_{2j
}+\frac{(1-\delta)^2}{4} \min[1, 2x_{1j} + 2x_{2j}] =
$$
$$
\frac{1+\delta}{2} \frac{1-\delta}{2} \cdot 2x_{1j} +  \frac{1+\delta}{2} \frac{1-\delta}{2} \cdot
2x_{2j} +  \frac{(1-\delta)^2}{4} \min[1, 2x_{1j} + 2x_{2j}]
$$
which is at least
$$
\frac{2-2\delta^2}{4} (x_{1j} + x_{2j}) + \frac{1-2\delta + \delta^2}{4} (x_{1j} + x_{2j}) \geq
(1-\delta) \frac{3}{4}  (x_{1j} + x_{2j}).
$$
\end{proof}

